Individual Closed Horocyclic Orbits on the Modular Surface

We track the trajectories of individual horocycles on the modular surface. Our tracking is constructive, and we thus \emph{effectively} establish topological transitivity and even line-transitivity for the horocyclic flow. We also describe homotopy class jumps that occur under continuous deformation of horocycles.

==> 4arXiv/markmac.tex <==
\newcommand{\aac}{\mbox{A-A-C} }
\newcommand{\bce}{\begin{center}}
\newcommand{\ece}{\end{center}}
%\newcommand{\vsp}[1]{\vspace{#1truein}}
\newcommand{\matSp}[3]{\left( \begin{array}{cc}
{#1}\Spm & {#2}\Spm \\
{#3}/\Spm & -{#1}\Spm \end{array} \right) }
\newcommand{\mat}[4]{\left( \begin{array}{cc}
{#1} & {#2} \\
{#3} & {#4} \end{array} \right) }
\newcommand{\alp}{{\alpha}}
\newcommand{\gamz}{\mbox{$\Gamma^0(p)$ }}
\newcommand{\bet}{{\beta}}
\newcommand{\gam}{{\gamma}}
\newcommand{\del}{{\delta}}
\newcommand{\pri}{^{\prime}}
\newcommand{\Si}[2]{\mbox{$\sigma^{#1}_{#2}$ }}
\newcommand{\Sim}[2]{\sigma^{#1}_{#2}}
\newcommand{\SLi}[1]{\mbox{$\sigma_L^{#1}$ }}
\newcommand{\SLim}[1]{\sigma_L^{#1}}
\newcommand{\pgroup}{\mbox{$\Gamma^*_p$ }}
\newcommand{\Ni}{\noindent}
\newcommand{\psurf}{\mbox{\ensuremath{\Gamma_p^* \backslash \mathcal H}}}
%\newcommand{\Sp}{\mbox{$\sqrt{p}$ }}
\newcommand{\Spm}{\sqrt{p}}
\newcommand{\Lpf}[2]{\mbox{$\frac{#1p \pm \Spm}{#2}$ }}
\newcommand{\Opf}[3]{\mbox{$\frac{#1 + \sqrt{#2}}{#3}$ }}
\newcommand{\matp}[4]{\left(      \begin{array}{cc}
{#1} & {#2}p^2 \\
{#3}p & {#4} \end{array} \right)}
\newcommand{\matpp}[4]{\left(      \begin{array}{cc}
{#1} & {#2}p \\
{#3} & {#4} \end{array} \right)}
\newcommand{\pqn}[1]{\mbox{$\frac{p_{#1}}{q_{#1}}$ }}
\newcommand{\abpn}[4]{\mbox{${#1}p_{#2} +{#3}p_{#4}$ }}
\newcommand{\abqn}[4]{\mbox{${#1}q_{#2} +{#3}q_{#4}$ }}
\newcommand{\abpqn}[4]{\mbox{$\frac{{#1}p_{#2} +
{#3}p_{#4}}{{#1}q_{#2} +
{#3}q_{#4}}$ }}
\newcommand{\pwfxd}{point-wise fixed }
\newcommand{\keq}[1]{\mbox{$x^2 - py^2 = #1$ }}
\newcommand{\hgq}{\mbox{$G_q$  }}
\newcommand{\eps}{\epsilon}
\newcommand{\sii}{\sigma}
\newcommand{\lqq}{\lambda_q}
\newcommand{\Gamq}{\mbox{\ensuremath{\Gamma_q} }}
\newcommand{\minusq}{\mbox{\ensuremath{G_q - \Gamq} }}
\newcommand{\qsurf}{\ensuremath{\Gamma_q \backslash {\mathcal H}}}
\newcommand{\Nn}{\mbox{${\mathcal N}$ }}
\newcommand{\Zz}{\mbox{${\mathbb Z}$ }}
\newcommand{\Qq}{\mbox{${\mathbb Q}$ }}
\newcommand{\qfield}{\ensuremath{Q(\lqq)}}
\newcommand{\gqsurf}{\ensuremath{G_q \backslash {\mathcal H}}}
\newcommand{\modsurf}{\ensuremath{\Gamma(1) \backslash {\mathcal H}}}
\newcommand{\fsurf}{\ensuremath{G_4  \backslash {\mathcal H}}}
\newcommand{\ssurf}{\ensuremath{G_6  \backslash {\mathcal H}}}
\newcommand{\modu}{\ensuremath{\Gamma(1)}}
\newcommand{\lqqq}{\ensuremath{\lambda_q}}
\newcommand{\gamq}{\Gamq}
\newcommand{\csurf}{\ensuremath{{\Gamma^\prime}\backslash {\mathcal H}} }
\newcommand{\theq}{\ensuremath{\Theta_q} }
\newcommand{\tsurf}{\ensuremath{\Theta_q \backslash {\mathcal H}}}
\newcommand{\MS}{\ensuremath{{\mathcal MS}} }
\newcommand{\lam}{\lambda}
\newcommand{\frq}{${\mathcal F}_{\Theta_q}$ }
\newcommand{\fsrq}{${\mathcal F}^*_{\Theta_q}$ }
\newcommand{\glam}{G_\lambda}
\newcommand{\hlam}{H_\lambda}
\newcommand{\sA}[1]{S^{a_{#1}}}
\newcommand{\wl}{\operatorname{wl}}
\newcommand{\len}{\operatorname{\ell}}
\newcommand{\glsurf}{\ensuremath{\glam \backslash {\mathcal H}} }
\newcommand{\hlsurf}{\ensuremath{\hlam \backslash {\mathcal H}} }
\newcommand{\niel}{{\mathcal N}}
\newcommand{\uhp}{{\mathcal H}}
\newcommand{\trr}{\operatorname{tr}}
\newcommand{\Trr}{\operatorname{Tr}}
\newcommand{\fll}{\operatorname{fl}}
\newcommand{\unit}{{\mathcal U}}
\newcommand{\mathcals}{{\mathcal S}}
\newcommand{\mathcalf}{{\mathcal F}}
\newcommand{\gamth}{\ensuremath{\Gamma_{\theta} }}
\newcommand{\gaminf}{\Gamma_{inf} }
\newcommand{\gamthsurf}{\ensuremath{\gamth \backslash {\mathcal H}} }
\newcommand{\gaminfsurf}{\ensuremath{\gaminf \backslash {\mathcal H}} }
\newcommand{\threesurf}{\ensuremath{\Gamma^3 \backslash {\mathcal H}} }
\newcommand{\xisurf}{\ensuremath{\varXi \backslash {\mathcal H}} }
\newcommand{\sphsurf}{\ensuremath{\Gamma (3) \backslash {\mathcal H}} }
\newcommand{\gammapr}{\ensuremath{\Gamma^{\prime}}}
\newcommand{\fre}{\mathcal{R}_\lam}
\newcommand{\klam}{_{k,\, \lam}}
\newcommand{\mathcalh}{$\mathcal{H}$ }
\newcommand{\mathcalp}{$\mathcal{P}$ }
\newcommand{\mathcalr}{$\mathcal{R}$ }
\renewcommand{\phi}{\varphi}
\renewcommand{\theta}{\vartheta}
\renewcommand{\Xi}{\varXi}\newcommand{\mathcali}{$\mathcal I$ }
\newcommand{\teich}{Teichm\"{u}ller }
\newcommand{\pee}[2]{P_{{#1}}^{{#2}}}
\newcommand{\gammathr}{\ensuremath{\Gamma (3)}}
\newcommand{\gammacu}{\ensuremath{\Gamma^3}}
\newcommand{\twogammacu}{\ensuremath{2\Gamma^3}}
\newcommand{\zsig}{\ensuremath{z_\sigma} }
\newcommand{\twogroup}{\ensuremath{\Gamma^2}}
\newcommand{\twosurf}{\ensuremath{\Gamma^2 \backslash \mathcal{H}}}
\newcommand{\gammaprsurf}{\ensuremath{\Gamma^{\prime} \backslash \mathcal{H}}}
\newcommand{\mma}{\textsc{Mathematica} }
\endinput

==> arXiv edition/markmac.tex <==
\newcommand{\aac}{\mbox{A-A-C} }
\newcommand{\bce}{\begin{center}}
\newcommand{\ece}{\end{center}}
%\newcommand{\vsp}[1]{\vspace{#1truein}}
\newcommand{\matSp}[3]{\left( \begin{array}{cc}
{#1}\Spm & {#2}\Spm \\
{#3}/\Spm & -{#1}\Spm \end{array} \right) }
\newcommand{\mat}[4]{\left( \begin{array}{cc}
{#1} & {#2} \\
{#3} & {#4} \end{array} \right) }
\newcommand{\alp}{{\alpha}}
\newcommand{\gamz}{\mbox{$\Gamma^0(p)$ }}
\newcommand{\bet}{{\beta}}
\newcommand{\gam}{{\gamma}}
\newcommand{\del}{{\delta}}
\newcommand{\pri}{^{\prime}}
\newcommand{\Si}[2]{\mbox{$\sigma^{#1}_{#2}$ }}
\newcommand{\Sim}[2]{\sigma^{#1}_{#2}}
\newcommand{\SLi}[1]{\mbox{$\sigma_L^{#1}$ }}
\newcommand{\SLim}[1]{\sigma_L^{#1}}
\newcommand{\pgroup}{\mbox{$\Gamma^*_p$ }}
\newcommand{\Ni}{\noindent}
\newcommand{\psurf}{\mbox{\ensuremath{\Gamma_p^* \backslash \mathcal H}}}
%\newcommand{\Sp}{\mbox{$\sqrt{p}$ }}
\newcommand{\Spm}{\sqrt{p}}
\newcommand{\Lpf}[2]{\mbox{$\frac{#1p \pm \Spm}{#2}$ }}
\newcommand{\Opf}[3]{\mbox{$\frac{#1 + \sqrt{#2}}{#3}$ }}
\newcommand{\matp}[4]{\left(      \begin{array}{cc}
{#1} & {#2}p^2 \\
{#3}p & {#4} \end{array} \right)}
\newcommand{\matpp}[4]{\left(      \begin{array}{cc}
{#1} & {#2}p \\
{#3} & {#4} \end{array} \right)}
\newcommand{\pqn}[1]{\mbox{$\frac{p_{#1}}{q_{#1}}$ }}
\newcommand{\abpn}[4]{\mbox{${#1}p_{#2} +{#3}p_{#4}$ }}
\newcommand{\abqn}[4]{\mbox{${#1}q_{#2} +{#3}q_{#4}$ }}
\newcommand{\abpqn}[4]{\mbox{$\frac{{#1}p_{#2} +
{#3}p_{#4}}{{#1}q_{#2} +
{#3}q_{#4}}$ }}
\newcommand{\pwfxd}{point-wise fixed }
\newcommand{\keq}[1]{\mbox{$x^2 - py^2 = #1$ }}
\newcommand{\hgq}{\mbox{$G_q$  }}
\newcommand{\eps}{\epsilon}
\newcommand{\sii}{\sigma}
\newcommand{\lqq}{\lambda_q}
\newcommand{\Gamq}{\mbox{\ensuremath{\Gamma_q} }}
\newcommand{\minusq}{\mbox{\ensuremath{G_q - \Gamq} }}
\newcommand{\qsurf}{\ensuremath{\Gamma_q \backslash {\mathcal H}}}
\newcommand{\Nn}{\mbox{${\mathcal N}$ }}
\newcommand{\Zz}{\mbox{${\mathbb Z}$ }}
\newcommand{\Qq}{\mbox{${\mathbb Q}$ }}
\newcommand{\qfield}{\ensuremath{Q(\lqq)}}
\newcommand{\gqsurf}{\ensuremath{G_q \backslash {\mathcal H}}}
\newcommand{\modsurf}{\ensuremath{\Gamma(1) \backslash {\mathcal H}}}
\newcommand{\fsurf}{\ensuremath{G_4  \backslash {\mathcal H}}}
\newcommand{\ssurf}{\ensuremath{G_6  \backslash {\mathcal H}}}
\newcommand{\modu}{\ensuremath{\Gamma(1)}}
\newcommand{\lqqq}{\ensuremath{\lambda_q}}
\newcommand{\gamq}{\Gamq}
\newcommand{\csurf}{\ensuremath{{\Gamma^\prime}\backslash {\mathcal H}} }
\newcommand{\theq}{\ensuremath{\Theta_q} }
\newcommand{\tsurf}{\ensuremath{\Theta_q \backslash {\mathcal H}}}
\newcommand{\MS}{\ensuremath{{\mathcal MS}} }
\newcommand{\lam}{\lambda}
\newcommand{\frq}{${\mathcal F}_{\Theta_q}$ }
\newcommand{\fsrq}{${\mathcal F}^*_{\Theta_q}$ }
\newcommand{\glam}{G_\lambda}
\newcommand{\hlam}{H_\lambda}
\newcommand{\sA}[1]{S^{a_{#1}}}
\newcommand{\wl}{\operatorname{wl}}
\newcommand{\len}{\operatorname{\ell}}
\newcommand{\glsurf}{\ensuremath{\glam \backslash {\mathcal H}} }
\newcommand{\hlsurf}{\ensuremath{\hlam \backslash {\mathcal H}} }
\newcommand{\niel}{{\mathcal N}}
\newcommand{\uhp}{{\mathcal H}}
\newcommand{\trr}{\operatorname{tr}}
\newcommand{\Trr}{\operatorname{Tr}}
\newcommand{\fll}{\operatorname{fl}}
\newcommand{\unit}{{\mathcal U}}
\newcommand{\mathcals}{{\mathcal S}}
\newcommand{\mathcalf}{{\mathcal F}}
\newcommand{\gamth}{\ensuremath{\Gamma_{\theta} }}
\newcommand{\gaminf}{\Gamma_{inf} }
\newcommand{\gamthsurf}{\ensuremath{\gamth \backslash {\mathcal H}} }
\newcommand{\gaminfsurf}{\ensuremath{\gaminf \backslash {\mathcal H}} }
\newcommand{\threesurf}{\ensuremath{\Gamma^3 \backslash {\mathcal H}} }
\newcommand{\xisurf}{\ensuremath{\varXi \backslash {\mathcal H}} }
\newcommand{\sphsurf}{\ensuremath{\Gamma (3) \backslash {\mathcal H}} }
\newcommand{\gammapr}{\ensuremath{\Gamma^{\prime}}}
\newcommand{\fre}{\mathcal{R}_\lam}
\newcommand{\klam}{_{k,\, \lam}}
\newcommand{\mathcalh}{$\mathcal{H}$ }
\newcommand{\mathcalp}{$\mathcal{P}$ }
\newcommand{\mathcalr}{$\mathcal{R}$ }
\renewcommand{\phi}{\varphi}
\renewcommand{\theta}{\vartheta}
\renewcommand{\Xi}{\varXi}\newcommand{\mathcali}{$\mathcal I$ }
\newcommand{\teich}{Teichm\"{u}ller }
\newcommand{\pee}[2]{P_{{#1}}^{{#2}}}
\newcommand{\gammathr}{\ensuremath{\Gamma (3)}}
\newcommand{\gammacu}{\ensuremath{\Gamma^3}}
\newcommand{\twogammacu}{\ensuremath{2\Gamma^3}}
\newcommand{\zsig}{\ensuremath{z_\sigma} }
\newcommand{\twogroup}{\ensuremath{\Gamma^2}}
\newcommand{\twosurf}{\ensuremath{\Gamma^2 \backslash \mathcal{H}}}
\newcommand{\gammaprsurf}{\ensuremath{\Gamma^{\prime} \backslash \mathcal{H}}}
\newcommand{\mma}{\textsc{Mathematica} }
\endinput
